V2W-BERT: A Framework for Effective Hierarchical Multiclass Classification of Software Vulnerabilities

Weaknesses in computer systems such as faults, bugs and errors in the architecture, design or implementation of software provide vulnerabilities that can be exploited by attackers to compromise the security of a system. Common Weakness Enumerations (CWE) are a hierarchically designed dictionary of software weaknesses that provide a means to understand software flaws, potential impact of their exploitation, and means to mitigate these flaws. Common Vulnerabilities and Exposures (CVE) are brief low-level descriptions that uniquely identify vulnerabilities in a specific product or protocol. Classifying or mapping of CVEs to CWEs provides a means to understand the impact and mitigate the vulnerabilities. Since manual mapping of CVEs is not a viable option, automated approaches are desirable but challenging. We present a novel Transformer-based learning framework (V2W-BERT) in this paper. By using ideas from natural language processing, link prediction and transfer learning, our method outperforms previous approaches not only for CWE instances with abundant data to train, but also rare CWE classes with little or no data to train. Our approach also shows significant improvements in using historical data to predict links for future instances of CVEs, and therefore, provides a viable approach for practical applications. Using data from MITRE and National Vulnerability Database, we achieve up to 97% prediction accuracy for randomly partitioned data and up to 94% prediction accuracy in temporally partitioned data. We believe that our work will influence the design of better methods and training models, as well as applications to solve increasingly harder problems in cybersecurity.

==> OLD-2introduction.tex <==
% Cybersecurity
%AP: edited 1/28/2021

\section{Introduction}
\label{sec:intro}


Mapping Common Vulnerabilities and Exposures (CVE)\footnote{\url{https://cve.mitre.org/cve/}} to Common Weakness Enumeration (CWE)\footnote{\url{https://cwe.mitre.org}} --  is an important but challenging problem in cyber-security~ \citep{Martin2008, Jimenez2016, Cruzes2017}. CVE is a list of common identifiers for publicly known cyber-security vulnerabilities. 
%A unique identifier is associated with a vulnerability or exposure through a system of CVE Numbering Authorities (CNAs) across the world.
CVEs provide classification and categorization of vulnerabilities, attacks, faults, and reference points for data exchange to standardize and make interoperable cyber-security products and services, and to enable information collection and sharing. CWE is a community-developed, formal list of common software weaknesses, such as: Buffer Overflows, Structure and Validity Problems, Handler Errors, and Authentication Errors.  CWE provides a common language to describe software security weaknesses, a metric for assessing software security tools addressing the vulnerabilities, and  a baseline standard for weakness identification, mitigation, and prevention efforts. 

\begin{figure}[htpb]
 \centering
 \includegraphics[width=\linewidth]{images/v2W-BERT-Overview.pdf}
 \caption{An illustration of the problem space that spans abundant as well as rare instances that need to be mapped. The cumulative number of CVEs are plotted along Y-axis (log scale) for a CWEs in different buckets for two time periods: 1999-2017 and 2018-2020. The proposed framework (\textsc{V2W-BERT}) also addresses the rare instances effectively.}
 \label{fig:Overview}
\end{figure}


CVEs are assigned to CWEs manually by security experts, and this process is not scalable. Security professionals require a precise understanding of the description of the vulnerabilities and the structure and definition of weakness. With the increasing number of CVE reports every year, it will be intractable to categorize these, maintaining quality and precision.
Therefore, algorithms and software tools %utility 
for automated processing of CVEs are critical necessities for optimal mitigation of known vulnerabilities and threats~\citep{Wu2010}. 

There are some key challenges in automating this process. Mitre categorized the common weaknesses into 916 CWEs based on Research Concepts~\footnote{https://cwe.mitre.org/data/definitions/1000.html}. These CWEs maintain a hierarchical structure that allows for multiple levels of abstraction. CWEs located at higher levels of the structure provide a broad overview of a vulnerability type and can have many CWEs associated with them. Each vulnerability can belong to several weaknesses at different levels of the hierarchy. The National Vulnerabilities Dataset (NVD) categorized most of the CVEs among currently available vulnerabilities (82K out of 137K). However, not all CWE definitions are used in practice, and the NVD utilizes only a cross-section of the CWEs (about 124)~\footnote{https://nvd.nist.gov/vuln/categories}. Interestingly, most of the weaknesses are rarely used and have a small number of vulnerability reports associated with them.

The hierarchical relationships and  the scarcity of vulnerability reports in most CWE categories make the automation of this problem challenging.
To illustrate, consider a practical scenario of classifying the vulnerabilities based on past data $(1999-2017)$ and predicting future years $(2018-2020)$. Fig~\ref{fig:CWEdist} shows the distribution of the number of CVEs associated with different CWEs. 
%distribution of different CWEs based on how many CVEs are associated with each weakness. 
Most CWEs ($84$ out of $124$) have fewer than $100$ cases, and some have no associated examples. Based on these  CVEs counts, we grouped the CWEs as frequent, rare, and completely unforeseen cases. Fig~\ref{fig:CVEdist} shows distribution of the vulnerabilities in the aforementioned groups in years $(1999-2017)$ and $(2018-2020)$. 
Historically rare cases have been appearing more frequently in  recent years, and classifying these is the primary challenge faced by any method.  

\begin{figure}[htpb]
    %\centering
    \begin{subfigure}[l]{0.5\linewidth}
        \includegraphics[width=\linewidth]{images/CWEdistribution.png}
        \caption{CWE distribution}
        \label{fig:CWEdist}
    \end{subfigure}%
    \begin{subfigure}[r]{0.5\linewidth}
        \centering
        \includegraphics[width=\linewidth]{images/CVEdistribution.png}
        \caption{CVE distribution}
        \label{fig:CVEdist}
    \end{subfigure}
    
    \caption{a) Distribution of CWEs in the year (1999-2017) by number of CVEs associated in each CWE, b) Log scale plot of total number of CVEs occurs frequently and rarely in year (1999-2017) and (2018-2020).}
    \label{fig:CWEdistribution}
\end{figure}

Existing approaches~\citep{na2016study, aota2020automation, neuhaus2010security, rehman2012software} for the automatic classification of this problem  %However, most of the existing approaches~
use only a few CWE categories, ignoring rare vulnerability cases,  and do not consider hierarchy at all.
Some recent authors~\citep{aghaei2019threatzoom, han2017learning,nakagawa2019character} use Neural Networks and word embedding-based methods to process vulnerability reports, and showed improved performance in related classification tasks.

In this work we propose a novel powerful Transformer-based learning algorithm~\citep{vaswani2017attention}, %based learning algorithm
V2W\textsubscript{BERT}, that outperforms related approaches in classifying vulnerabilities for both rare and frequent cases.  
The Bidirectional Encoder Representations from Transformers (BERT)~\citep{devlin2018bert} is designed to pre-train deep bidirectional representations from unlabeled text by jointly conditioning on both the left and right sides of the context of a text token  during the training phase. 
BERT is trained on a large text corpus, learning a deeper and intimate understanding of how language works, which is useful for downstream language processing tasks. The pre-trained BERT model can be fine-tuned with additional custom layers, and can be employed to create state-of-the-art models for a wide range of Natural Language Processing (NLP) tasks~\citep{devlin2018bert,sun2019fine}.  

The use of such a powerful model to transfer knowledge to the security domain and use it for classification purposes has been beneficial. The primary contributions of the proposed V2W\textsubscript{BERT} algorithm can be summarized as follows:

%changes here by sid
\begin{enumerate}
    \item This is the first Transformer based machine learning approach to classify CVEs into CWEs. 
    Our proposed model takes advantage of both labeled and unlabeled CVE descriptions.
    V2W\textsubscript{BERT} uses pre-trained BERT models in a siamese~\citep{chicco2020siamese} architecture to predict links between CVEs and CWEs. 
    Rare and unforeseen vulnerabilities are classified thanks to the transfer learning procedure. The Reconstruction Decoder enforces that the pre-trained model on unsupervised data is not compromised by the overfitting of the link prediction task.
    
    %\item In this work, all $124$ available CWEs from NVD are used along with the hierarchical relationships among them.
    
    \item We are the first in formalizing the problem of associating multiple-weakness definition into a single vulnerability (multi-class) as a link prediction task.
    The hierarchical relationships among the CWEs are also incorporated during training and prediction.
    Unlike the traditional classification based methods, adding a new CWE definition later requires no change in the model architecture.
    
    \item The use of BERT based transfer learning outperforms related approaches in all types of CWEs (both rare and frequently occurring). Additionally, the proposed method can classify completely unforeseen types of CWEs to some extent. This also gives us the potential to detect if and when a new CWE definition is necessary.
    
    \item We simulate a  challenging real-world scenario in our experiments where future mappings (2018-2020) are predicted based on past years' (1999-2017) data. 
    For frequently occurring cases, V2W\textsubscript{BERT} predicts future associations with $89\%-98\%$ accuracy for precise and relax prediction. (Definitions for these two types of prediction are provided later.)  For rarely occurring CVEs, the proposed method achieves $48\%-76\%$ prediction accuracy, which is $10\%$ to $15\%$ more than the existing approach.
    We predict the CWEs of a vulnerability to the finer-granularity (root to the leaf node), where the user can control the precision.
\end{enumerate}

Our paper is organized as follows. 
In Section~\ref{sec:background} related work and preliminaries of  BERT are discussed. Section~\ref{sec:method} describes the proposed V2W\textsubscript{BERT} algorithm in detail, and   Section~\ref{sec:ablation} discusses  how each algorithmic component is optimized for performance. Section~\ref{sec:comparison} shows comparative performance with related approaches, and this is  followed by discussion and concluding remarks.

% The Common Weakness Enumeration Specification (CWE) provides a common language of discourse for discussing, finding and dealing with the causes of software security vulnerabilities as they are found in code, design, or system architecture. Each individual CWE represents a single vulnerability type. CWE is currently maintained by the MITRE Corporation. A detailed CWE list is currently available at the MITRE website~\footnote{https://cwe.mitre.org/data/definitions/1000.html}; this list provides a detailed definition for each individual CWE.

% All individual CWEs are held within a hierarchical structure that allows for multiple levels of abstraction. CWEs located at higher levels of the structure (i.e. Configuration ) provide a broad overview of a vulnerability type and can have many children CWEs associated with them. CWEs at deeper levels in the structure (i.e. Cross Site Scripting ) provide a finer granularity and usually have fewer or no children CWEs. 
% %The image to the right represents a portion of the overall CWE structure, the red boxes represent the CWEs being used by NVD.

% NVD integrates CWE into the scoring of CVE vulnerabilities by providing a cross section of the overall CWE structure. NVD analysts score CVEs using CWEs from different levels of the hierarchical structure. This cross section of CWEs allows analysts to score CVEs at both a fine and coarse granularity, which is necessary due to the varying levels of specificity possessed by different CVEs.

% NVD is using CWE as a classification mechanism that differentiates CVEs by the type of vulnerability they represent. 


% \textbf{Stuff about BERT}
% BERT stands for Bidirectional Encoder Representations from Transformers. It is designed to pre-train deep bidirectional representations from unlabeled text by jointly conditioning on both left and right context. As a result, the pre-trained BERT model can be fine-tuned with just one additional output layer to create state-of-the-art models for a wide range of NLP tasks.”

% This pre-training step is half the magic behind BERT’s success. This is because as we train a model on a large text corpus, our model starts to pick up the deeper and intimate understandings of how the language works. This knowledge is the swiss army knife that is useful for almost any NLP task.

% Third, BERT is a “deep bidirectional” model. Bidirectional means that BERT learns information from both the left and the right side of a token’s context during the training phase.

% To learn more about the BERT architecture and its pre-training tasks, then you may like to read the below article:

==> preamble.tex <==
\usepackage{geometry}
% \geometry{letterpaper,textwidth=350pt,textheight=680pt,tmargin=60pt,
%             left=72pt,footskip=24pt,headsep=18pt,headheight=14pt}
\RequirePackage{amsmath}
%\usepackage{amssymb}
\usepackage{textcase}
\usepackage{soul}
\usepackage{indentfirst}

\newcommand{\eps}{\varepsilon}
\newcommand{\kron}{\otimes}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\trace}{trace}
\DeclareMathOperator{\tvec}{vec}
\DeclareMathOperator{\rank}{rank}
\DeclareMathOperator{\tspan}{span}
\DeclareMathOperator*{\minimize}{minimize}
\DeclareMathOperator*{\maximize}{maximize}
\DeclareMathOperator{\subjectto}{subject\ to}

\newcommand{\mat}[1]{\boldsymbol{#1}}
\renewcommand{\vec}[1]{\boldsymbol{\mathrm{#1}}}
\newcommand{\vecalt}[1]{\boldsymbol{#1}}

\newcommand{\conj}[1]{\overline{#1}}

\newcommand{\normof}[1]{\|#1\|}
\newcommand{\onormof}[2]{\|#1\|_{#2}}

\newcommand{\MIN}[2]{\begin{array}{ll} \displaystyle \minimize_{#1} & {#2} \end{array}}
\newcommand{\MINone}[3]{\begin{array}{ll} \displaystyle \minimize_{#1} & {#2} \\ \subjectto & {#3} \end{array}}
\newcommand{\OPTone}{\MINone}
\newcommand{\MINthree}[5]{\begin{array}{ll} \displaystyle \minimize_{#1} & {#2} \\ \subjectto & {#3} \\ & {#4} \\ & {#5} \end{array}}

\newcommand{\MAX}[2]{\begin{array}{ll} \displaystyle \maximize_{#1} & {#2} \end{array}}
\newcommand{\MAXone}[3]{\begin{array}{ll} \displaystyle \maximize_{#1} & {#2} \\ \subjectto & {#3} \end{array}}


\newcommand{\itr}[2]{#1^{(#2)}}
\newcommand{\itn}[1]{^{(#1)}}

\newcommand{\prob}{\mathbb{P}}
\newcommand{\probof}[1]{\prob\left\{ #1 \right\}}

\newcommand{\pmat}[1]{\begin{pmatrix} #1 \end{pmatrix}}
\newcommand{\bmat}[1]{\begin{bmatrix} #1 \end{bmatrix}}
\newcommand{\spmat}[1]{\left(\begin{smallmatrix} #1 \end{smallmatrix}\right)}
\newcommand{\sbmat}[1]{\left[\begin{smallmatrix} #1 \end{smallmatrix}\right]}

\newcommand{\RR}{\mathbb{R}}
\newcommand{\CC}{\mathbb{C}}

\providecommand{\eye}{\mat{I}}
\providecommand{\mA}{\ensuremath{\mat{A}}}
\providecommand{\mB}{\ensuremath{\mat{B}}}
\providecommand{\mC}{\ensuremath{\mat{C}}}
\providecommand{\mD}{\ensuremath{\mat{D}}}
\providecommand{\mE}{\ensuremath{\mat{E}}}
\providecommand{\mF}{\ensuremath{\mat{F}}}
\providecommand{\mG}{\ensuremath{\mat{G}}}
\providecommand{\mH}{\ensuremath{\mat{H}}}
\providecommand{\mI}{\ensuremath{\mat{I}}}
\providecommand{\mJ}{\ensuremath{\mat{J}}}
\providecommand{\mK}{\ensuremath{\mat{K}}}
\providecommand{\mL}{\ensuremath{\mat{L}}}
\providecommand{\mM}{\ensuremath{\mat{M}}}
\providecommand{\mN}{\ensuremath{\mat{N}}}
\providecommand{\mO}{\ensuremath{\mat{O}}}
\providecommand{\mP}{\ensuremath{\mat{P}}}
\providecommand{\mQ}{\ensuremath{\mat{Q}}}
\providecommand{\mR}{\ensuremath{\mat{R}}}
\providecommand{\mS}{\ensuremath{\mat{S}}}
\providecommand{\mT}{\ensuremath{\mat{T}}}
\providecommand{\mU}{\ensuremath{\mat{U}}}
\providecommand{\mV}{\ensuremath{\mat{V}}}
\providecommand{\mW}{\ensuremath{\mat{W}}}
\providecommand{\mX}{\ensuremath{\mat{X}}}
\providecommand{\mY}{\ensuremath{\mat{Y}}}
\providecommand{\mZ}{\ensuremath{\mat{Z}}}
\providecommand{\mLambda}{\ensuremath{\mat{\Lambda}}}
\providecommand{\mSigma}{\ensuremath{\mat{\Sigma}}}
\providecommand{\mPbar}{\bar{\mP}}

\providecommand{\ones}{\vec{e}}
\providecommand{\va}{\ensuremath{\vec{a}}}
\providecommand{\vb}{\ensuremath{\vec{b}}}
\providecommand{\vc}{\ensuremath{\vec{c}}}
\providecommand{\vd}{\ensuremath{\vec{d}}}
\providecommand{\ve}{\ensuremath{\vec{e}}}
\providecommand{\vf}{\ensuremath{\vec{f}}}
\providecommand{\vg}{\ensuremath{\vec{g}}}
\providecommand{\vh}{\ensuremath{\vec{h}}}
\providecommand{\vi}{\ensuremath{\vec{i}}}
\providecommand{\vj}{\ensuremath{\vec{j}}}
\providecommand{\vk}{\ensuremath{\vec{k}}}
\providecommand{\vl}{\ensuremath{\vec{l}}}
\providecommand{\vm}{\ensuremath{\vec{l}}}
\providecommand{\vn}{\ensuremath{\vec{n}}}
\providecommand{\vo}{\ensuremath{\vec{o}}}
\providecommand{\vp}{\ensuremath{\vec{p}}}
\providecommand{\vq}{\ensuremath{\vec{q}}}
\providecommand{\vr}{\ensuremath{\vec{r}}}
\providecommand{\vs}{\ensuremath{\vec{s}}}
\providecommand{\vt}{\ensuremath{\vec{t}}}
\providecommand{\vu}{\ensuremath{\vec{u}}}
\providecommand{\vv}{\ensuremath{\vec{v}}}
\providecommand{\vw}{\ensuremath{\vec{w}}}
\providecommand{\vx}{\ensuremath{\vec{x}}}
\providecommand{\vy}{\ensuremath{\vec{y}}}
\providecommand{\vz}{\ensuremath{\vec{z}}}
\providecommand{\vpi}{\ensuremath{\vecalt{\pi}}}

\providecommand{\vlambda}{\ensuremath{\vecalt{\lambda}}}


%%added by me
\usepackage{tikz}
\usepackage{forest}
\usetikzlibrary{arrows.meta, calc}
\usetikzlibrary{positioning,arrows,chains}
\usepackage{tikz-qtree}
\usetikzlibrary{trees}
\usetikzlibrary{matrix,fit}

\usepackage{hyperref}       % hyperlinks
\hypersetup{
    colorlinks=true,
    linkcolor=blue,
    filecolor=magenta,      
    urlcolor=blue,
    citecolor=blue,
}

\usepackage{url}        
\usepackage{graphicx}
\usepackage{multirow}
\usepackage{caption}
\usepackage{subcaption}
\usepackage{svg}

\newcommand{\payAttention}[3]{\textcolor{#1}{{{#2}: {#3}}}}
% \renewcommand{\payAttention}[3]{}
\newcommand{\todo}[1]{\payAttention{red}{TODO}{#1}}
\newcommand{\xSays}[2]{\payAttention{blue}{#1 Says}{#2}}
\newcommand{\Alex}[1]{{\xSays{Alex}{#1}}}
\newcommand{\Sid}[1]{\xSays{Siddhartha}{#1}}
\newcommand{\Mahantesh}[1]{\xSays{Mahantesh}{#1}}
\newcommand{\Edoardo}[1]{\xSays{Edoardo}{#1}}
%\newcommand{\tamal}[1]{\xSays{Tamal}{#1}}

